Program Machine Policy: Addressing Long-Horizon Tasks by Integrating Program Synthesis and State Machines

Deep reinforcement learning (deep RL) excels in various domains but lacks generalizability and interpretability. On the other hand, programmatic RL methods (Trivedi et al., 2021; Liu et al., 2023) reformulate RL tasks as synthesizing interpretable programs that can be executed in the environments. Despite encouraging results, these methods are limited to short-horizon tasks. On the other hand, representing RL policies using state machines (Inala et al., 2020) can inductively generalize to long-horizon tasks; however, it struggles to scale up to acquire diverse and complex behaviors. This work proposes the Program Machine Policy (POMP), which bridges the advantages of programmatic RL and state machine policies, allowing for the representation of complex behaviors and the address of long-term tasks. Specifically, we introduce a method that can retrieve a set of effective, diverse, and compatible programs. Then, we use these programs as modes of a state machine and learn a transition function to transition among mode programs, allowing for capturing repetitive behaviors. Our proposed framework outperforms programmatic RL and deep RL baselines on various tasks and demonstrates the ability to inductively generalize to even longer horizons without any fine-tuning. Ablation studies justify the effectiveness of our proposed search algorithm for retrieving a set of programs as modes.

==> figure/inductive_curves_only.tex <==
\begin{figure}
    \centering
    \includegraphics[trim=80 0 100 0,clip,width=\columnwidth]{figure/exp_figure/ig.pdf}
    \caption{Inductive Generalization}
    \label{fig:ig}
    %\vspace{-0.1cm}
    \caption[]{
        \small 
        \textbf{Inductive generalization performance.}
        We evaluate and report the performance drop in the testing environments with an extended horizon, where the x-axis is the extended horizon length compared to the horizon of the training environments, and the y-axis is the performance drop in percentage.
        Our proposed framework can inductively generalize to longer horizons without any fine-tuning.
    }
\end{figure}

==> figure/stage1_CEM.tex <==
\begin{figure*}
\begin{subfigure}{.39\textwidth}
  \centering
  % include first image
  \includegraphics[width=.95\linewidth]{figure/models/stage_2_CEM.pdf}  
  \caption{\textbf{Cross Entropy Method (CEM)}}
  \label{fig:stage2_cem}
\end{subfigure}
\begin{subfigure}{.59\textwidth}
  \centering
  % include second image
  \includegraphics[width=.95\linewidth]{figure/models/stage_2_Evaluation_Function.pdf} 
  \caption{\textbf{Evaluation Function}}
  \label{fig:stage2_eval_func}
\end{subfigure}
\vfill
\begin{subfigure}{.44\textwidth}
  \centering
  % include third image
  \includegraphics[width=.99\linewidth]{figure/models/stage_2_CEM_Diversity.pdf}  
  \caption{\textbf{CEM+diversity}}
  \label{fig:stage2_cem_div}
\end{subfigure}
\begin{subfigure}{.52\textwidth}
  \centering
  % include fourth image
  \includegraphics[width=.99\linewidth]{figure/models/stage_2_CEM_Diversity_Compatibility.pdf}  
  \caption{\textbf{CEM+diversity+compatibility}}
  \label{fig:stage2_cem_div_com}
\end{subfigure}
\caption{
   \small 
        Searching for a set of effective and reusable program embedding that can be decoded to programs of various skills.
        (a): Using the Cross-Entropy Method to search for a program with high execution reward in the learned program embedding space.
        (b): The program evaluation function $G$ is used during program search.
        (c): Conducting CEM multiple times and selecting the best program. The \textit{diversity multiplier} is used to avoid identical results and increase diversity among multiple CEM searches.
        (d): Searching for a diverse set of program embeddings that are compatible with each other in terms of execution order $SQ_1$ and $SQ_2$.
}
\label{fig:stage1_cem}
\end{figure*}

==> table/ablation_one_program.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}
\centering
\caption{\textbf{Comparing CEM and CEM+diversity.}
The accumulated rewards of programs retrieved by CEM and CEM+diversity. The mean and standard deviation are evaluated over five random seeds. CEM+diversity outperforms CEM with significantly smaller standard deviations across 8 out of 10 tasks, highlighting the effectiveness and stability of CEM+diversity.}
\label{tab:karel_Karel_hard}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
  Method &
  \begin{tabular}[c]{@{}c@{}}\textsc{Four}\\ \textsc{Corner}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textsc{Top}\\ \textsc{Off}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textsc{Clean}\\ \textsc{House}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textsc{Stair}\\ \textsc{Climber}\end{tabular} &
  \textsc{Harvester} &
  \textsc{Maze} &
  \begin{tabular}[c]{@{}c@{}}\textsc{Door}\\ \textsc{Key}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textsc{One}\\ \textsc{Stroke}\end{tabular} &
  \textsc{Seeder} &
  \textsc{Snake} \\ 
\midrule
CEM & 0.45 $\pm$ 0.40 & 0.81 $\pm$ 0.07 & 0.18 $\pm$ 0.14 & \textbf{1.00} $\pm$ 0.00 & 0.45 $\pm$ 0.28 & \textbf{1.00} $\pm$ 0.00 & \textbf{0.50} $\pm$ 0.00 & \textbf{0.65} $\pm$ 0.19 & 0.51 $\pm$ 0.21 & 0.21 $\pm$ 0.15\\

\begin{tabular}[c]{@{}c@{}}CEM+diversity\end{tabular} & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{0.37} $\pm$ 0.06 & \textbf{1.00} $\pm$ 0.00 & \textbf{0.80} $\pm$ 0.07 & \textbf{1.00} $\pm$ 0.00 & \textbf{0.50} $\pm$ 0.00 & 0.62 $\pm$ 0.01 & \textbf{0.69} $\pm$ 0.07 & \textbf{0.36} $\pm$ 0.02 \\ 
\bottomrule
\end{tabular}
}
\end{table*}

==> table/karel_karel_hard_scoreboard_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage{booktabs}
\begin{table}
\centering
\caption{\textbf{\textsc{Karel} and \textsc{Karel-Hard} Performance.} Mean return and standard deviation of all methods across the \textsc{Karel} and \textsc{Karel-Hard} problem set, evaluated over five random seeds. As the table shows, POMP outperforms LEAPS and HPRL on most \textsc{Karel} and \textsc{Karel Hard} tasks, except \textsc{OneStroke} and \textsc{Snake}, which need good long-term planning abilities. One thing to notice is that, unlike \textsc{Karel-Long}, \textsc{Karel} and \textsc{Karel-Hard} do not have per-action cost in design, so for POMP here, we did not let it learn to terminate but gave a maximum mode program execution number. Therefore, the whole policy will stop when this number is reached, or the task is solved.}
\label{tab:karel_Karel_hard_POMP}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
  Method &
  \begin{tabular}[c]{@{}c@{}}Four\\ Corner\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Top\\ Off\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Clean\\ House\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Stair\\ Climber\end{tabular} &
  Harvester &
  Maze &
  \begin{tabular}[c]{@{}c@{}}Door\\ Key\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}One\\ Stroke\end{tabular} &
  Seeder &
  Snake \\ 
  \midrule
DRL & 0.29 $\pm$ 0.05 & 0.32 $\pm$ 0.07 & 0.00 $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & 0.90 $\pm$ 0.10 & \textbf{1.00} $\pm$ 0.00 & 0.48 $\pm$ 0.03 & \textbf{0.89} $\pm$ 0.04 & 0.96 $\pm$ 0.02 & \textbf{0.67} $\pm$ 0.17 \\
LEAPS & 0.45 $\pm$ 0.40 & 0.81 $\pm$ 0.07 & 0.18 $\pm$ 0.14 & \textbf{1.00} $\pm$ 0.00 & 0.45 $\pm$ 0.28 & \textbf{1.00} $\pm$ 0.00 & 0.50 $\pm$ 0.00 & 0.65 $\pm$ 0.19 & 0.51 $\pm$ 0.21 & 0.21 $\pm$ 0.15\\
HPRL (5) & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & 0.50 $\pm$ 0.00 & 0.80 $\pm$ 0.02 & 0.58 $\pm$ 0.07 & 0.28 $\pm$ 0.11\\

\midrule
\begin{tabular}[c]{@{}c@{}}POMP\end{tabular} & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & \textbf{1.00} $\pm$ 0.00 & 0.62 $\pm$ 0.01 & \textbf{0.97} $\pm$ 0.02 & 0.36 $\pm$ 0.02 \\ 
\bottomrule 
\end{tabular}
}
\end{table}

==> table/karel_long_scoreboard.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage{booktabs}

% \begin{table*}[t]
% \centering
% \caption{\textbf{\textsc{Karel-Long} Performance.} 
% Mean return and standard deviation of all methods across the \textsc{Karel-Long} problem set, evaluated over five random seeds. 
% By learning a program machine policy with a set of effective, diverse, and compatible mode programs, our proposed framework achieves the best mean reward in \textsc{Seesaw}, \textsc{UP-N-Down}, and \textsc{Farmer}. It also performs competitively in \textsc{Inf-DoorKey} and \textsc{Inf-Harvester}.}
% \label{tab:karel_long}
% \resizebox{0.85\textwidth}{!}{%
% \begin{tabular}{cccccc}
% \toprule
%    Method
%  &
%   \textsc{Seesaw} &
%   \textsc{Up-N-Down} &
%   \textsc{Farmer} &
%   \textsc{Inf-DoorKey}  &\begin{tabular}[c]{@{}c@{}} \textsc{Inf-Harvester} \end{tabular} 
% \\ 
% \midrule

% CEM $\times|M|$                             & 0.31 $\pm$ 0.18 & 0.88 $\pm$ 0.12 & 0.22 $\pm$ 0.00 & 0.39 $\pm$ 0.46  &0.56 $\pm$ 0.12 
% \\
% CEM+diversity top $k$, $k=|M|$            & 0.09 $\pm$ 0.11 & 0.72 $\pm$ 0.36 & 0.23 $\pm$ 0.00 & 0.92$\pm$ 0.01 &0.71 $\pm$ 0.02
% \\
% CEM+diversity $\times|M|$                 & 0.47 $\pm$ 0.39 & 0.76 $\pm$ 0.31 & 0.24 $\pm$ 0.03 & 0.89 $\pm$ 0.02  &0.66 $\pm$ 0.07 
% \\ 
% \midrule
% DRL                                                                          & 0.00 $\pm$ 0.00& 0.00 $\pm$ 0.00& 0.55 $\pm$ 0.16& \textbf{0.97} $\pm$ 0.01 &0.45 $\pm$ 0.03 
% \\
% Random Transition                                                         & 0.08 $\pm$ 0.03& 0.03 $\pm$ 0.17& 0.09 $\pm$ 0.03& 0.13 $\pm$ 0.08 &0.14 $\pm$ 0.07 
% \\
% PSMP                                                                         & 0.25 $\pm$ 0.39& 0.00 $\pm$ 0.00& 0.58 $\pm$ 0.06& \textbf{0.97} $\pm$ 0.01 &0.59 $\pm$ 0.06 
% \\
% MMN                                                                          & 0.10 $\pm$ 0.00& 0.00 $\pm$ 0.00& 0.57 $\pm$ 0.12 & 0.87 $\pm$ 0.05 & 0.41 $\pm$ 0.10 
% \\
% LEAPS                                                                        & 0.10 $\pm$ 0.10& 0.38 $\pm$ 0.05& 0.15 $\pm$ 0.06& 0.10 $\pm$ 0.04 &0.06 $\pm$ 0.06 
% \\
% HPRL                                                                    & 0.00 $\pm$ 0.00& 0.00 $\pm$ 0.00& 0.40 $\pm$ 0.18& 0.15 $\pm$ 0.21 &\textbf{0.85} $\pm$ 0.06
% \\ 
% \midrule
% POMP (Ours) & \textbf{0.90} $\pm$ 0.02& \textbf{0.97} $\pm$ 0.00& \textbf{0.88} $\pm$ 0.01& 0.91$\pm$ 0.01 &0.67 $\pm$ 0.03 \\ 
% \bottomrule

% \end{tabular}%
% }
% \end{table*}

==> table/program2.tex <==
\begin{figure*}[ht]
\centering
\begin{mdframed}[frametitle=Karel Programs]
\begin{subfigure}[t]{0.90\textwidth}

\centering
\textbf{\textsc{Farmer}}

{
\begin{subfigure}[t]{0.32\textwidth}
Mode 1
\begin{lstlisting}
DEF run m( 
    pickMarker 
    REPEAT R=0 r( 
        pickMarker 
        move 
        turnRight 
        move 
        move 
        turnLeft 
        move 
        move 
        turnRight 
        move 
        turnLeft 
        move 
        move 
        pickMarker 
        move 
        turnLeft 
        move 
        move 
        pickMarker 
        move 
        turnLeft 
        move 
        move 
        pickMarker 
        move 
        r) 
    m)


\end{lstlisting}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
Mode 2
\begin{lstlisting}
DEF run m( 
    turnRight 
    move 
    putMarker 
    turnRight 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    m)

\end{lstlisting}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
Mode 3
\begin{lstlisting}
DEF run m( 
    turnRight 
    move 
    turnRight 
    putMarker 
    pickMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    m)

\end{lstlisting}
\end{subfigure}
}

{
\begin{subfigure}[t]{0.32\textwidth}
Mode 4
\begin{lstlisting}
DEF run m( 
    REPEAT R=17 r( 
        IF c( not c( rightIsClear c) c) i( 
            putMarker 
            move 
            i) 
        r) 
    m)
\end{lstlisting}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
Mode 5
\begin{lstlisting}
DEF run m( 
    putMarker 
    pickMarker 
    turnRight 
    move 
    pickMarker 
    turnRight 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    pickMarker 
    putMarker 
    move 
    m)
\end{lstlisting}
\end{subfigure}

}
\end{subfigure}
% \end{mdframed}
% \end{figure*}

% \begin{figure*}[h]
% \centering
% \begin{mdframed}
\begin{subfigure}[t]{0.90\textwidth}

\centering
\textbf{\textsc{Inf-Doorkey}}

{
\begin{subfigure}[t]{0.32\textwidth}
Mode 1
\begin{lstlisting}
DEF run m( 
    IFELSE c( noMarkersPresent c) i( 
        move 
        putMarker 
        i) 
    ELSE e( 
        pickMarker 
        putMarker 
        e) 
    m)

\end{lstlisting}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
Mode 2
\begin{lstlisting}
DEF run m( 
    IF c( noMarkersPresent c) i( 
        move 
        move 
        move 
        IF c( noMarkersPresent c) i( 
            move 
            REPEAT R=1 r( 
                move 
                turnLeft 
                r) 
            i) 
        i) 
    IF c( noMarkersPresent c) i( 
        move 
        REPEAT R=1 r( 
            move 
            REPEAT R=1 r( 
                move 
                r) 
            r) 
        i) 
    m)
\end{lstlisting}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
Mode 3
\begin{lstlisting}
DEF run m( 
    putMarker 
    pickMarker 
    IF c( not c( markersPresent c) c) i( 
        move 
        i) 
    WHILE c( noMarkersPresent c) w( 
        IFELSE c( markersPresent c) i( 
            turnLeft 
            i) 
        ELSE e( 
            move 
            turnRight 
            e) 
        w) 
    m)

\end{lstlisting}
\end{subfigure}
}

{
\begin{subfigure}[t]{0.32\textwidth}
Mode 4
\begin{lstlisting}
DEF run m( 
    putMarker 
    turnLeft 
    pickMarker 
    move 
    turnLeft 
    IFELSE c( markersPresent c) i( 
        move 
        turnLeft 
        i) 
    ELSE e( 
        move 
        e) 
    m)
\end{lstlisting}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
Mode 5
\begin{lstlisting}
DEF run m( 
    turnRight 
    IF c( leftIsClear c) i( 
        turnLeft 
        i) 
    putMarker 
    IF c( leftIsClear c) i( 
        turnLeft 
        i) 
    pickMarker 
    move 
    IF c( leftIsClear c) i( 
        turnLeft 
        i) 
    putMarker 
    move 
    IF c( leftIsClear c) i( 
        turnLeft 
        i) 
    pickMarker 
    move 
    m)
\end{lstlisting}
\end{subfigure}
% \begin{subfigure}[t]{0.32\textwidth}
% Mode 1
% \begin{lstlisting}
% DEF run m( 
%     REPEAT R=5 r( 
%         move 
%         WHILE c( noMarkersPresent c) w( 
%             move 
%             w) 
%         putMarker 
%         r)
%     m)

% \end{lstlisting}
% \end{subfigure}
}

\end{subfigure}
% \end{mdframed}
% \end{figure*}

% \begin{figure*}[h]
% \centering
% \begin{mdframed}


\end{mdframed}
\caption[\method\\ Karel Tasks Synthesized Programs]{\textbf{Example programs on Karel-Long tasks: \textsc{Farmer} and \textsc{Inf-Doorkey}.} The programs with best rewards out of all random seeds are shown.
}
\label{fig:karel_program_examples_farmer_infDoorKey}
\end{figure*}




==> text/broader_impacts.tex <==
\section*{Impact Statements}
%Yet, extending LEAPS to such domains can potentially lead to some negative societal impacts. For example, our framework can still capture unintended bias during learning or suffer from adversarial attacks. Furthermore, policies deployed in the real world can create great economic impact by causing job losses in some sectors. Therefore, we would encourage further work to investigate the biases, safety issues, and potential economic impacts to ensure that the deployment in the field does not cause far-reaching, negative societal impacts.

Our work introduces the Program Machine Policy (POMP), a novel framework that combines programmatic RL and state machine policies, enabling autonomous agents to represent complex behaviors and address long-term tasks. POMP demonstrates significant potential in automating laborious or risky tasks, enhancing the efficiency and safety of autonomous systems. While offering promising societal benefits, we acknowledge the importance of addressing ethical considerations, including potential biases inherited from training data or adversarial attacks. 
Ongoing research in the field of responsible AI and fairness in machine learning aims to mitigate these biases, and we acknowledge the importance of continuous efforts to ensure that AI systems, including POMP, adhere to ethical standards and contribute positively to society.



%The introduction of Program Machine Policies (POMPs) in our work represents a significant advancement in addressing the challenges of generalizability and interpretability within deep reinforcement learning (RL). As we contemplate the broader impacts of our proposed framework, it is imperative to consider both the potential benefits and ethical considerations associated with its deployment in real-world applications.

%On the positive front, POMPs offer a unique synthesis of programmatic RL and state machine policies, providing a promising avenue for representing complex behaviors and tackling long-term tasks. By introducing a method to retrieve effective, diverse, and compatible programs, we enable autonomous learning agents to generalize their knowledge to diverse scenarios without the need for extensive fine-tuning. This capability has far-reaching implications for automation in various domains, potentially revolutionizing tasks that are laborious, arduous, or pose risks to humans. The prospect of enhancing the efficiency and safety of autonomous systems stands out as a key societal benefit, aligning with the overarching goal of advancing the field of machine learning.

%However, as with any technological advancement, it is crucial to address potential ethical considerations. The introduction of autonomous learning agents, especially those capable of representing complex behaviors, raises concerns about the potential biases and ethical implications embedded in the training data or expert demonstrations. Similar to the example provided, the biases of expert demonstrators can be inherited by the POMPs, potentially leading to sub-optimal, unsafe, or discriminatory behaviors. Ongoing research in the field of responsible AI and fairness in machine learning aims to mitigate these biases, and we acknowledge the importance of continuous efforts to ensure that AI systems, including POMPs, adhere to ethical standards and contribute positively to society.

%In conclusion, while our work introduces a powerful framework with the potential to transform the landscape of deep RL, it is essential to approach its deployment with a mindful consideration of ethical implications. By actively engaging in ongoing discussions and research related to fairness, bias mitigation, and responsible AI, we aspire to contribute to the development of AI systems that not only excel in performance but also adhere to ethical principles, fostering a positive impact on society.
